Accelerating Spatio-Textual Queries with Learned Indices

Efficiently computing spatio-textual queries has become increasingly important in various applications that need to quickly retrieve geolocated entities associated with textual information, such as in location-based services and social networks. To accelerate such queries, several works have proposed combining spatial and textual indices into hybrid index structures. Recently, the novel idea of replacing traditional indices with ML models has attracted a lot of attention. This includes works on learned spatial indices, where the main challenge is to address the lack of a total ordering among objects in a multidimensional space. In this work, we investigate how to extend this novel type of index design to the case of spatio-textual data. We study different design choices, based on either loose or tight coupling between the spatial and textual part, as well as a hybrid index that combines a traditional and a learned component. We also perform an experimental evaluation using several real-world datasets to assess the potential benefits of using a learned index for evaluating spatio-textual queries.

==> Preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}

% \noindent \emph{The R-Tree family of indices.} Most traditional spatio-textual indices are \mnote{based on the R-tree~\cite{Guttman1984} for the spatial indexing part. Recall that an R-tree organizes a hierarchy of nested $d$-dimensional rectangles. Each node represents the MBR of its children or, for leaf nodes, the MBR of its contained geometries. The number of entries per node (excluding the root) is between a lower bound $m$ and a maximum capacity $M$. Query execution in R-trees starts from the root. MBRs in any visited node are tested for intersection against a search region. Qualifying entries are recursively visited until the leaf level or until no further overlaps are found. Several paths may be probed, because multiple sibling entries could overlap with the search region.} R*-Trees~\cite{beckmann1990r} are an improved variant of R-Trees, which introduces optimizations on the area, margin and overlap of the nodes' MBRs.

\noindent \emph{The R-Tree family of indices.} Most traditional spatio-textual indices employ an R-tree~\cite{Guttman1984} or the more efficient R*-Tree~\cite{beckmann1990r} for indexing spatial information. Recall that an R-tree organizes a hierarchy of nested $d$-dimensional {\em Minimum bounding Rectangles} (MBRs). Apart from the root node, the capacity of every inner or leaf node ranges between a lower bound $m$ and a maximum number $M$ of entries. Query execution starts from the root and recursively traverses the subtree of a node if its MBR intersects with the query region.
\fixme{Figure~\ref{fig:r-tree} depicts an example of an R-Tree, with two entries per node. {\em Do we need it? Everyone should know what R-tree looks like.}}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.65\linewidth]{Figures/R-Tree.eps}
    \caption{The R-Tree}
    \label{fig:r-tree}
\end{figure}

\noindent \emph{Inverted indices.}
Inverted indices are widely used in textual databases for keyword-based search, e.g., in web search engines. An inverted index stores elements from a content (e.g., words) and maps them to a list of document IDs where they can be found. Figure~\ref{fig:inv_index} depicts an example of an inverted index over the keywords used by a set of  spatio-textual objects; each keyword $w$ lists the subset of objects that include it.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\linewidth]{Figures/Inverted_index.eps}
    \caption{Example of an inverted index.}
    \label{fig:inv_index}
\end{figure}

\noindent \emph{Signatures.}
Text signatures~\cite{faloutsos1984signature} are essentially Bloom filters and are used in signature files to quickly rule out documents that do not contain a certain set of words (false positives are possible). There are two methods for signature extraction, based on hashing and superimposed coding respectively. In this work, we associate a \textit{bitmap} to each spatio-textual object as the signature of its keywords. Specifically, each keyword in the corpus corresponds to a single bit in the bitmap. If the object includes a keyword, the corresponding bit is set, as in the example illustrated in Figure~\ref{fig:bitmap}.
%Apparently, the text represented by this bitmap contains the words ``pizza'', ``fish'' and ``bar''.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/bitmap.eps}
    \caption{Bitmap representing an object's keywords.}
    \label{fig:bitmap}
\end{figure}

\noindent \emph{The IR$^2$-Tree.}
The IR$^2$-tree~\cite{defelipe2008icde} is a state-of-the-art \mnote{traditional?} spatio-textual index, tailored to answer Boolean queries (i.e., BWQ/\fixme{BRQ?} and B$kQ$). Essentially, each node of the R*-Tree, apart from its children MBRs, is also enhanced with keyword-related information. \fixme{Since it is a rather old index, it takes under consideration during construction the HDD page size; it should be able to fit all node data within a single page. Thus it employs keyword signatures, with a fixed number of bits. -> {\em Rephrased:} To hold all node data in a single disk page, it employs signatures of a small, fixed size, even for a large corpus of keywords.}  This, of course, can result in reduced pruning efficiency due to many false positives in upper tree levels. Although multi-level superimposed coding~\cite{sacks1983two} can be applied for those signatures, false positives cannot be avoided. Since our suggested indices in this work are all memory-based, we are not constrained by the signature size. Thus, to eliminate false positives, in our implementation of IR$^2$-trees we simply associate a bitmap over the entire corpus to each node, which directly indicates the presence of keywords in its subtree, as exemplified in Figure~\ref{fig:ir2tree}. 
%Notice that, each node and raw spatio-textual object within its leaves are associated with a specific bitmap.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/IR2-Tree.eps}
    \caption{The IR$^2$-Tree}
    \label{fig:ir2tree}
\end{figure*}

\noindent \emph{RSMI.}
The recently introduced Recursive Spatial Model Index (RSMI)~\cite{qi2020effectively}, employs a rank space-based ordering technique similar to an R-Tree packing strategy~\cite{qi2018theoretically}. This establishes an ordering over point data and groups those points into \textit{blocks}, before applying a space-filling curve. As in most ML-based indices, RSMI employs a feed forward neural network and learns a function $f$ that maps curve values to blocks' rankings. For scalability, RSMI applies a recursive, $k-d-tree$-like~\cite{bentley1975multidimensional} partitioning strategy and trains smaller models separately for each partition. Thus, the trained models have to estimate ranks on fewer objects, which ensures higher accuracy. \mnote{The MBR of each node (model), is also kept and can be probed during querying to enhance pruning}. 

Figure~\ref{fig:rsmi} exemplifies an RSMI \fixme{against another dataset?}. The data is initially partitioned (\fixme{leftmost part of the image -> enumerate?}) according to a maximum size \mnote{$N$} allowed per partition. Once a partition ends up with less than $N$ objects, it is no longer split. A space-filling curve (e.g., $z$-order curve) over the centroids of the resulting partitions derives the ordering and a model is trained to match each object to a partition. Then, for each object, the trained model is used to predict the partition number and the final partitions are generated (\fixme{middle part of the image -> enumerate?}). If one of them exceeds max size \mnote{$N$}, it is further partitioned (\fixme{rightmost part of the image-> enumerate?}). For each resulting partition we train a leaf model that maps its objects to blocks. During query processing, we first use the higher level models to estimate the partition(s) to further evaluate. Then, upon reaching a leaf model, we estimate the block range to evaluate, taking under consideration the errors of the trained models. \fixme{Explain error in a sentence? Symbol $\epsilon$ ?}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/RSMI.eps}
    \caption{The RSMI Index.}
    \label{fig:rsmi}
\end{figure*}


==> Related.tex <==
\section{Related Work}
\label{sec:related}

\fixme{This Section could be moved before Conclusions? What we need in our analysis is contained in Preliminaries. Otherwise, we could merge both sections into `Background and Related Work'.}

\noindent \emph{Spatio-Textual Indices.} The increasing amount of generated spatio-textual objects has motivated research on hybrid queries combining location-based predicates with keyword search. A special category of hybrid queries are \textit{Boolean queries}, which include the Boolean window query (a special case of the Boolean range query) and the Boolean $k$NN query, as discussed in~\cite{chen2013pvldb}.

Efficient evaluation of boolean spatio-textual queries can be carried out by hybrid index structures that simultaneously partition the data in both domains, spatially and textually. \mnote{Essentially, this implies combining a spatial index structure (e.g., R-tree~\cite{Guttman1984}, Quadtree~\cite{samet1984quadtree}) or a space-filling curve~\cite{sagan2012space} with a textual index (e.g., inverted file~\cite{zobel2006inverted}, signature file~\cite{faloutsos1984signature}). Depending on their form, the resulting variants can be characterized either as {\em spatial-first} or {\em textual-first} indices \cite{christoforaki2011cikm}. One of the most fundamental and characteristic ones is the IR-tree \cite{cong2009vldb,zhisheng2011tkde}, which extends the R-tree by augmenting the contents of each node with a pointer to an inverted file, thus indexing terms and documents contained in its sub-tree. Several other hybrid spatio-textual indices extending the R-tree (or R$^*$-tree) have been proposed, such as the IR$^2$-tree \cite{defelipe2008icde}, the KR$^*$-Tree \cite{hariharan2007ssdbm}, SKI \cite{cary2010ssdbm} and S2I \cite{rocha2011ssd}, while methods based on space filling curves include SF2I \cite{chen2006sigmod} and SFC-QUAD \cite{christoforaki2011cikm}}.

\noindent \emph{Learned Indices.} Recently, a new family of indices has emerged, leveraging the potential of machine learning to estimate the order of an object in a sorted list of objects. If such a total ordering exists, this essentially replaces the traditional index structure, since neighboring objects will be closely located. The first learned index approaches were one-dimensional, where a total ordering of the objects is rather straightforward. Though, research has expanded to multiple dimensions, where ordering the objects is more challenging. 

Learned indices can be categorized to {\em immutable} (i.e., do not support insertions/deletions) and {\em mutable}. The pioneering approach in~\cite{kraska2018case} introduced RMI, a one-dimensional immutable learned index approach, which replaces B-Tree index structures with deep learning models in a hierarchical manner. Other immutable, but multidimensional learned indices include~\cite{wang2019learned}, which introduces Z-order Model (ZM) index, a data-driven index structure that combines the $z$-order space-filling curve with the staged learning model to learn the distribution of the data. Tsunami~\cite{ding2020tsunami} introduces a learned index that automatically estimates its parameters based on the given dataset and workload in the presence of correlated and skewed data. 

Regarding mutable learned indices, ALEX~\cite{ding2020alex} is a one-dimensional method addressing various learned index issues when applied on workloads that contain point lookups, short range queries, inserts, updates, and deletes. The mutable multidimensional learned index in~\cite{davitkova2020ml} generalizes the idea of the iDistance~\cite{jagadish2005idistance} scaling method and uses the scaled ordering in combination with a two-layer learned index, to answer multidimensional queries. LISA~\cite{li2020lisa} proposes a learned index structure for spatial data, which consists of a mapping function that maps spatial keys into 1-dimensional mapped values, a learned shard prediction function that partitions the mapped space into shards, and a series of local models that organize shards into pages. Finally, RSMI~\cite{qi2020effectively} is a spatial learned index that employs a rank space based ordering technique based on the $z$-order space-filling curve to establish an ordering of point data and eliminate large gaps in the resulting cumulative distribution function. All learned index methods that we examine in this paper are based on RSMI, extending its applicability on spatio-textual data.
